Towards Debiasing Fact Verification Models

Fact verification requires validating a claim in the context of evidence. We show, however, that in the popular FEVER dataset this might not necessarily be the case. Claim-only classifiers perform competitively with top evidence-aware models. In this paper, we investigate the cause of this phenomenon, identifying strong cues for predicting labels solely based on the claim, without considering any evidence. We create an evaluation set that avoids those idiosyncrasies. The performance of FEVER-trained models significantly drops when evaluated on this test set. Therefore, we introduce a regularization method which alleviates the effect of bias in the training data, obtaining improvements on the newly created test set. This work is a step towards a more sound evaluation of reasoning capabilities in fact verification models.

==> sections/92_app_examp.tex <==
\section{Examples from the Symmetric Dataset}
\label{sec:db_examp}



\begin{table*}[t]
\small
\begin{tabular}{c|l|l|c}
\textbf{Source} & \multicolumn{1}{c|}{\textbf{Claim}} & \multicolumn{1}{c|}{\textbf{Evidence}} & \textbf{Label} \\ \hline \hline
\textbf{\textsc{Original}} & \begin{tabular}[c]{@{}l@{}}Tim Roth is an English actor.\\ \end{tabular} & \begin{tabular}[c]{@{}l@{}}Timothy Simon Roth (born 14 May 1961) is\\ an English actor and director.\end{tabular} & \textsc{Support} \\ \hline
\textbf{\textsc{Generated}} & \begin{tabular}[c]{@{}l@{}}Tim Roth is an American actor.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Timothy Simon Roth (born 14 May 1961) is \\an American actor and director.\end{tabular} & \textsc{Support} \\ \hline \hline
\textbf{\textsc{Original}} & \begin{tabular}[c]{@{}l@{}}Aristotle spent time in Athens.\end{tabular} & \begin{tabular}[c]{@{}l@{}}At seventeen or eighteen years of age,\\ he joined Plato's Academy in Athens and\\ remained there until the age of thirty-seven (c. 347 BC) .\end{tabular} & \textsc{Support} \\ \hline
\textbf{\textsc{Generated}}& \begin{tabular}[c]{@{}l@{}}Aristotle did not visit Athens.\end{tabular} & \begin{tabular}[c]{@{}l@{}}At seventeen or eighteen years of age, \\ he missed the opportunity to join Plato's Academy\\ in Athens and never visited the place.\end{tabular} & \textsc{Support} \\ \hline \hline
\textbf{\textsc{Original}} & \begin{tabular}[c]{@{}l@{}}Telemundo is a English-language \\television network.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Telemundo (teleˈmundo)  is an American Spanish-language\\ terrestrial television network owned by Comcast through the\\ NBCUniversal division NBCUniversal Telemundo Enterprises.\end{tabular} & \textsc{Refute} \\ \hline
\textbf{\textsc{Generated}} & \begin{tabular}[c]{@{}l@{}}Telemundo is a Spanish-language\\ television network.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Telemundo (teleˈmundo) is an American English-language\\ terrestrial television network owned by Comcast through the\\ NBCUniversal division NBCUniversal Telemundo Enterprises.\end{tabular} & \textsc{Refute} \\ \hline \hline
\textbf{\textsc{Original}} & \begin{tabular}[c]{@{}l@{}}Magic Johnson did not \\play for the Lakers.\end{tabular} & \begin{tabular}[c]{@{}l@{}}He played point guard for the Lakers for 13 seasons.\end{tabular} & \textsc{Refute} \\ \hline
\textbf{\textsc{Generated}} & Magic Johnson played for the Lakers. & He played for the Giants and no other team. & \textsc{Refute} \\ \hline \hline
\end{tabular}
\caption{Examples of cases from the Symmetric Dataset}
\label{tab:symm_examples}
\end{table*}


\tabref{tab:symm_examples} describes some examples of cases created for the Symmetric Dataset.
